Towards Efficient Neuro-Symbolic AI: From Workload Characterization to Hardware Architecture

The remarkable advancements in artificial intelligence (AI), primarily driven by deep neural networks, are facing challenges surrounding unsustainable computational trajectories, limited robustness, and a lack of explainability. To develop next-generation cognitive AI systems, neuro-symbolic AI emerges as a promising paradigm, fusing neural and symbolic approaches to enhance interpretability, robustness, and trustworthiness, while facilitating learning from much less data. Recent neuro-symbolic systems have demonstrated great potential in collaborative human-AI scenarios with reasoning and cognitive capabilities. In this paper, we aim to understand the workload characteristics and potential architectures for neuro-symbolic AI. We first systematically categorize neuro-symbolic AI algorithms, and then experimentally evaluate and analyze them in terms of runtime, memory, computational operators, sparsity, and system characteristics on CPUs, GPUs, and edge SoCs. Our studies reveal that neuro-symbolic models suffer from inefficiencies on off-the-shelf hardware, due to the memory-bound nature of vector-symbolic and logical operations, complex flow control, data dependencies, sparsity variations, and limited scalability. Based on profiling insights, we suggest cross-layer optimization solutions and present a hardware acceleration case study for vector-symbolic architecture to improve the performance, efficiency, and scalability of neuro-symbolic computing. Finally, we discuss the challenges and potential future directions of neuro-symbolic AI from both system and architectural perspectives.

==> Sections/6_Hardware.tex <==
\section{Case Study: Hardware Acceleration of Vector-Symbolic Architecture}
\label{sec:hardware}

%\blue{Add a transition paragraph/subsection from profiling insight to hardware acceleration, and mention use VSA as a case study to show co-design; tie VSA with NVSA workflow; Two-level transition: profiling - hardware; VSA kernel - operator.}

This section presents a programmable hardware accelerator for VSA, one of the essential component of the neuro-symbolic system. Building on the detailed analysis discussed previously, we develop a design method that overcomes computational inefficiencies arising from executing the vector-symbolic component on CPUs and GPUs (refer to Sec.~\ref{sec:results}). We particularly provide a hardware solution that involves: (1) an energy-efficient dataflow with heterogeneous arithmetic units that can flexibly execute binding, bundling, and distance computation---the key operations used in any vector-symbolic kernel, (2) a distributed memory system employing near-memory computing to enhance scalability and memory performance, (3) compressed storage of symbolic operators to reduce the memory footprint of vector codebooks, and (4) a tiled design for vector-symbolic units to minimize data movement and optimize computational efficiency. These features collectively enable a highly efficient and scalable vector-symbolic hardware accelerator that significantly outperforms traditional processing platforms.

We next present an overview of the accelerated vector-symbolic operations (Sec.~\ref{subsec:vsa_ops}), the accelerator's architecture (Sec.~\ref{subsec:accelerator_dataflow}), and its programming methodology (Sec.~\ref{subsec:accelerator_control}). 

%This section presents our method for VSA acceleration, including the architecture (Sec.~\ref{subsec:accelerator_dataflow}) and programming methodology (Sec.~\ref{subsec:accelerator_control}). The proposed accelerator aims to overcome the computational inefficiencies arising from executing VSA on traditional platforms (e.g., GPU), specifically by providing a hardware solution that includes: (1) heterogeneous arithmetic units tailored to the diverse computational requirements of VSA kernels, (2) a distributed memory system employing near-memory computing to enhance scalability and performance, (3) compressed storage of symbolic operators to reduce the memory footprint of vector codebooks, and (4) a tiled design for vector-symbolic units to minimize data movement and optimize computational efficiency. These features collectively enable a highly efficient and scalable VSA hardware accelerator that significantly outperforms traditional processing platforms.

\subsection{Vector-Symbolic Kernel Operations}
\label{subsec:vsa_ops}
%\blue{binding/bunding/distance/etc, profile at kernel-level, not operator-level, to design hardware for VSA, we need to understand VSA operator}

In the vector-symbolic kernel, computational elements, such as scalars and objects, are represented using high-dimensional holographic vectors, often referred to as hypervectors, which can be manipulated by a set of four algebraic operations: (1) binding, or element-wise multiplication, which creates a new hypervector that is quasi-orthogonal (dissimilar) to its constituents; (2) bundling, or element-wise addition, which combines hypervectors using element-wise majority count; (3) permutation, which rearranges the elements of a hypervector to preserve its order within a sequence; (4) scalar multiplication, which scales hypervector elements with a scalar weight. The similarity between vectors is measured using a distance metric, such as the dot product. These operations collectively form a mathematical framework for implementing various cognitive functions tailored for VSA operations (Sec.~\ref{subsec:nvsa-model})~\cite{kleyko2022vector}.
 % including the backend of NVSA

\subsection{Accelerator Architecture}
\label{subsec:accelerator_dataflow}

Shown in Fig.~\ref{fig:hpu_arch} is the proposed architecture, which consists of three subsystems: (1) memory and codebook-generation subsystem (MCG), (2) vector-symbolic operations subsystem (VOP), and (3) distance computation subsystem (DC). A control unit is used to decode instructions and determine control configurations. A description of these subsystems and their internal operations are presented below.
%, (4) systolic array-based neural engine (SN), and (5) a global controller unit (CTRL). %A control unit is used to decode instructions and determine control configurations. 
%Fig.~\ref{fig:hpu_arch} depicts these subsystems and their internal modules. 
 

% \noindent
\textbf{MCG Subsystem.} This subsystem is distributed across multiple tiles, with each tile comprising four functional modules: a local memory (SRAM), a logic unit implementing cellular automata with rule 90 (CA-90)~\cite{kleyko2021cellular}, a register file (CA-90 RF), and a query register (QRY). Vectors loaded from the local SRAM are processed exclusively within the tile's logic to leverage near-memory computing. The SRAMs are initialized with randomly generated atomic vectors (i.e., codebooks) used for symbolic encoding. The dimension of these vectors is constrained by the size of the physical datapth; therefore, we utilize a ``folding'' mechanism to support extended vector dimensions. CA-90 is integral to this mechanism, utilizing XOR and shift operations to generate new random vectors on-the-fly~\cite{kleyko2021cellular}. This design significantly reduces the memory footprint, as only seed folds need to be stored in the local SRAMs. CA-90 RF is a register file that temporarily stores newly generated folds to minimize redundant activations of CA-90. The QRY register holds query data required for similarity computation, an essential component of VSA. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{Figs/hpu_arch.pdf}
	\caption{The proposed hardware architecture for VSA acceleration.}
	\label{fig:hpu_arch}
 \vspace{-1em}
\end{figure}

% \noindent
\textbf{VOP Subsystem.} The VOP subsystem implements key VSA operations, used to construct distributed perceptual representations and perform symbolic reasoning computations. It consists of five logic units: a binding unit (BIND), a multiplying unit (MULT), a bundling unit (BND), a register file (BND RF), and a sign unit (SGN). BIND connects to a local buffer storing vectors and is to used to execute the binding operations over these vectors. The superposition of binded vectors is implemented in BND through element-wise addition (bundling). BIND and BND utilize different data representations, with BIND using binary and BND using integer formats. MULT manages the conversion from binary to integer formats and also performs element-wise scalar multiplication, an essential operation for neuro-symbolic encoding. Integer folds outputted from BND can be temporarily stored in BND RF for continuous superposition or converted to binary through SGN for transfer over the global vector-symbolic datapath. 

% \noindent
\textbf{DC Subsystem.} This subsystem handles operations for distance computation and nearest neighbor search, and it comprises three critical logic units: POPCNT, DSUM RF, and ARGMAX. POPCNT evaluates the popcount of the difference between two vectors; it executes element-wise XOR operations followed by an addition operation to compute the difference between the number of $1$'s and the number of $0$'s in the difference vector. As POPCNT operates on partial vectors due to vector folding, its output also represents a partial distance quantity. Hence, DSUM RF facilitates distance accumulation over multiple partial vectors, distributing distance computations across multiple independently controllable registers. The resulting distance data is then communicated to ARGMAX, which manages the search for the nearest neighbor vector based on the transferred distance values.

\subsection{Accelerator Control Methods}
\label{subsec:accelerator_control}

The configuration of the different modules as described above exhibits a pipelined architecture that consists of seven pipeline stages, with each stage associated with a certain type of operation (Fig.~\ref{fig:control_method}). Such a pipelined configuration motivates the search for programming methods that improves resource utilization while equipping with control over performance tradeoffs. To perform this study, we particularly examine two control methods for this accelerator: \emph{single-operation-per-cycle} (SOPC) and \emph{multiple-operations-per-cycle} (MOPC).

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{Figs/pipeline_stages.pdf}
	\caption{VSA accelerator's pipeline stages and operation types.}
	\label{fig:control_method}
 \vspace{-1em}
\end{figure}


SOPC simplifies programming and reduces power consumption since only one pipeline stage switches during each cycle. However, this approach increases runtime, making it unsuitable for high-throughput applications. Conversely, MOPC enables pipeline stages to perform operations simultaneously, thus increasing the number of operations per cycle (OPC). However, MOPC leads to increased power consumption, and furthermore, it requires a complex mapping framework (a compiler) to analyze program dependencies and optimize control activities. MOPC is better suited for high-throughput applications that require a balance between runtime and power consumption. 

\noindent\textbf{Analyzing Control Methods.} We compare SOPC and MOPC by the analyzing the mapping of a widely used VSA algorithm referred to as \emph{resonator network}~\cite{frady2020resonator}. This algorithm takes as input a composed vector (which may represent a visual scene involving multiple objects as in the RPM problem) and seeks to factorize the vector into its constituent factors. Comparison between SOPC and MOPC is performed with respect to runtime and power consumption, measured while executing this algorithm at various complexity levels (number of factors). 

Fig.~\ref{fig:SOPC_MOPC} illustrates the results of this study. We observe that MOPC achieves lower runtime in comparison with SOPC, and that the speed-up gained by using MOPC increases from $1.8$ to $2.3$. However, using MOPC also increases power consumption compared to SOPC. The percentage of increased power by using MOPC grows from $44\%$ to $57\%$ as the complexity increases; see Fig.~\ref{fig:SOPC_MOPC}(b). 

\noindent\textbf{Adopting MOPC.} We optimize the control-flow of our design based on MOPC as it offers two major advantages. First, MOPC provides the capability to speed up the execution of a given task, as opposed to SOPC. This is especially important when multiple heterogeneous tasks need to be executed simultaneously, e.g., layered 
% NVSA 
cognition frameworks. Second, the speed-up gain can be flexibly configured based on power-consumption constraints. Consider the case of executing a six-factor resonator network using MOPC. If the speed-up is decreased from $2.3$ to $2.0$, the average power consumption decreases from $9.3$ mW to $8.0$ mW. In fact, we could aim to decrease the speed-up further until it converges to that of SOPC; that is $1.0$, achieving a reduced power consumption of only $4.0$ mW. In other words, SOPC is considered a special case of MOPC. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=\columnwidth]{Figs/SOPC_MOPCS.pdf}
	\caption{Demonstration of the accelerator's behavior and performance tradeoffs when two control methods (SOPC and MOPC) are used to execute the resonator network algorithm: (a) runtime results, and (c) power-consumption results.}
	\label{fig:SOPC_MOPC}
 \vspace{-1em}
\end{figure}

\begin{figure}[!b]
 \vspace{-1em}
	\centering
	\includegraphics[width=0.93\columnwidth]{Figs/MPOC_ISA.pdf}
	\caption{The \emph{Instruction Word} format adopted in the proposed design. }
	\label{fig:MPOC_ISA}
\end{figure}

\noindent\textbf{Accelerator Instruction Format.} 
To realize the MOPC control method, we design an instruction-set architecture that employs a wide-word macro format, referred to as \emph{Instruction Word}. Similar to a Very-Large Instruction Word (VLIW), a single \emph{Word} consists of multiple operations, except that these operations are sequential in the pipelined dataflow and not parallel like VLIW architectures. As shown in Fig.~\ref{fig:MPOC_ISA}, the \emph{Word} format consists of seven \texttt{Type} fields, used to specify the operations to be executed in seven pipelined stages of HPU, and an \texttt{OP\_PARAM} field, used to configure all or specific \texttt{Type} operations. This approach offers a high degree of flexibility and is commonly used with domain-specific processors. Details on the instruction fields and compiler optimization are omitted due to lack of space. 



==> Sections/6_Optimization.tex <==
\section{Optimization Solutions}
\label{sec:optimization}

% ToDo: a table summarizing software and hardware optimization techniques, to improve which metrics.
This section presents the optimization solutions for neuro-symbolic, including software (Sec.~\ref{subsec:opt_sw}), system (Sec.~\ref{susbec:opt_sparsity}-\ref{subsec:opt_parallelism}), architecture (Sec.~\ref{subsec:opt_arch}), and technology (Sec.~\ref{subsec:opt_tech}) methods, to improve its performance and efficiency.

\subsection{Software: Model Compression and Efficient Factorization}
\label{subsec:opt_sw}
Quantization of neuro and symbolic components can reduce memory and data communication overhead and improve neuro-symbolic system efficiency. For example, we apply 8-bit integer quantization to neuro and symbolic computations in NVSA, and achieve $\sim$4$\times$ memory footprint and energy reduction, while maintaining 98.7\% cognitive reasoning accuracy on RAVEN task~\cite{zhang2019raven} (FP32 baseline has 98.8\% accuracy). By contrast, GPT-4~\cite{gpt4} and neuro-only (ResNet~\cite{he2016deep}) models only reach 89.0\% and 53.4\% accuracy, respectively, even with much larger footprints. Additionally, we propose to leverage efficient factorization modules to quickly factorize symbolic vectors and replace the burdened codebook when decomposing an object vector, and achieve 71.4$\times$ memory footprint reduction and 8.1$\times$ latency reduction compared to vector codebook, while maintaining 98.8\% RAVEN accuracy.

\colorbox{brown!30}{\textbf{Optimization 1:}} \textit{Model compression (e.g., quantization and pruning) and efficient factorization of neuro and symbolic components can reduce memory and data movement overhead without sacrificing cognitive reasoning accuracy.}
% Software: Quantization on neural and vector-symbolic operations, can employ fixed-point representation without sacrificing accuracy or performance; dynamic vector dimension adjustment; factorization to replace huge codebook. Neural quantization has been actively explored, but vector-symbolic quantization for binary and bipolar can be explored. 

\subsection{System: Neuro and Symbolic Component Sparsity}
\label{susbec:opt_sparsity}
Leveraging the high sparsity in neuro and symbolic components can greatly reduce the memory footprint and computation FLOPS. 
For example, for sparsity in NVSA (symbolic) (Fig.~\ref{fig:NVSA_sparsity}), the $n$$\times$$m$ sparse block code matrix contains only contains four non-zero values in every $m/4$ element for PMF-to-VSA transform ($m$=1024). We propose to store only the indices of non-zero values in a 32-bit (8-bit each) memory instead of storing all 1024 elements, and achieve 96.9$\times$ memory footprint reduction under same bit precision. Instead of $n$$\times$$m$ multiplications and additions, leveraging this sparsity requires only 4$n$ additions, resulting in a FLOPS decrease from 2.2M to 8.6K in NVSA. For sparsity in ZeroC (neuro), the input images are one-hot tuples of size 10$\times$16$\times$16$\times$64. We propose to store the indices of one-hot channels with 4-bit for each pixel, thus achieving 160$\times$ memory reduction. Additionally, the masks are also highly sparse given a threshold of sample iteration. After the threshold, the masks are $>$90\% sparse and can be stored in a compressed-spare row (CSR) format. Dedicated hardware design for sparse computation can further benefit the neuro-symbolic system efficiency~\cite{wu2022sparseloop,wu2023highlight,munoz2023flexagon}.
% In ZeroC, the sample iteration is 150 allowing a huge storage reduction for both images and masks. 

% As discussed in section V, both neural and symbolic operations can be sparse, and for a particular operation, the degree of sparsity can also vary. The difference in operation types and degree of sparsity call for different optimization techniques. We discuss two such techniques, one for sparsity in symbolic operations and one for sparsity in neural operations.

% Fig.~\ref{fig:NVSA_sparsity} shows the average sparsity in three stages of NVSA symbolic operations for each of the five attributes. It is observed that the average sparsity is very high, with the exception of position attribute in the S2 and S3 stages. Stage S1 is matrix multiplication between a PMF vector (1$\times$n) computed during the frontend and a binary sparse block-code matrix(n$\times$m). For m=1024, the codebook contains four non-zero values, one in every 256 elements. Codebook pre-processing can be highly memory and compute-efficient, storing only the indices of these four non-zero values in a 32-bit (8-bit each) memory instead of storing every 1024 elements. Even with the assumption of storing the original codebook with maximum quantization, up to 96.88$\times$ storage reduction is achieved. We just need four adders that will be responsible for adding the probability values to the output vector based on the non-zero codebook indices. Instead of m$\times$n multiplications and additions, we only require 4n additions, resulting in a decrease of FLOPS from 2.2M to 8.6K for the parameters used in NVSA. 

% Lets consider an example of sparsity in zeroC neural operations. The images in zeroC are one-hot tuples of size 10$\times$16$\times16$ and it increases 64 $\times$ to account for the ensemble. Instead of storing the whole image, we can only store the indices of one-hot channel using 4 bits for each pixel (16$\times$16), saving 160x storage overhead assuming maximum quantization. In addition to the images, the masks are also highly sparse given a threshold of sample iteration. After the threshold, the masks are more than 90\% sparse and can be stored in a compressed-spare row (CSR) format. In ZeroC, the sample iteration is 150 allowing a huge storage reduction for both images and masks. 


% \green{[Ritik:polish and compare with other compression formats]}

\colorbox{brown!30}{\textbf{Optimization 2:}} \textit{Sparsity-aware neuro and symbolic algorithm and architecture design can benefit memory footprint, communication overhead and computation FLOPS reduction.}
 % Existing sparsity-aware architectural paradigms focus on the optimization on the NN~\cite{jeong2023vegeta,kwon2018maeri,qin2020sigma,munoz2023flexagon}. Symbolic reasoning largely relies on bitwise operation ...
 % The data movement could be reduced by leveraging sparsity and weight reuse, e.g., the same submodel used for inference many times

\subsection{System: Parallelism and Adaptive Runtime Scheduling}
\label{subsec:opt_parallelism}
Enabling multi-level parallelism and adaptive workload scheduling on different compute substrates can alleviate hardware under-utilization and improve real-time performance. For example, we propose three-level parallelism for NVSA and PrAE, i.e., scene-level parallelism, attribute-level parallelism, and rule-level parallelism, and achieve 8.2$\times$ speedup on Xeon CPU and RTX 2080Ti system. With heterogeneous architecture, dynamic scheduling neuro and symbolic components on dedicated hardware substrates can further reduce latency.

\colorbox{brown!30}{\textbf{Optimization 3:}} \textit{Multi-level parallelism and adaptive workload scheduling of neuro and symbolic components can alleviate resource under-utilization and reduce runtime.} 
% Programmers (or better compilers) can optimize code at low-level to better leverage hardware resources.

\subsection{Architecture: Heterogeneous Hardware and Specialized PE}
\label{subsec:opt_arch}
Given the much greater heterogeneity in compute kernels of neuro-symbolic computing, it's highly desirable to design heterogeneous or reconfigurable hardware architecture, especially to efficiently support vector-symbolic operations and holographic vector representations in surging neuro-symbolic computing~\cite{kleyko2022vector}. For example, we implement a modified scale-out systolic architecture based on SCALE-Sim~\cite{samajdar2020systematic} with custom processing elements (PE) for vector-symbolic binding/bundling operations and observe 10.7$\times$ speedup. Additionally, caching reusable elements, such as codebook in NVSA and aggregated attribute distributions in PrAE, within multi-core network-on-chip (NoC), can alleviate bandwidth requirements. Leveraging high-bandwidth NoC for large intermediate values, such as neuro/symbolic interface in NVSA and PrAE and bidirectional inference in LNN, can reduce communication overhead. To further increase efficiency, it is also desirable to design circuits implementing compositional computational primitives from Sec.~\ref{subsec:operator}.

% can restrict the hardware performance due to restricted bandwidth of the traditional interconnection network. NoC tailored to NSAI workloads with high-bandwidth virtual channel~\cite{dally1992virtual} to mitigate potential network deadlocks and routers with large in/out buffers for large data movements such as NVSA/PrAE front-end to back-end and bidirectional inference in LNN. 

% results: speedup and memory footprint reduction after quantization on some workloads, without harming accuracy.


\colorbox{brown!30}{\textbf{Optimization 4:}} \textit{Heterogeneous or reconfigurable neuro/ symbolic architecture with efficient vector-symbolic units and high-bandwidth NoC can improve system performance.}
% Hardware: Caching the necessary element on-chip, and leveraging a high-bandwidth network-on-chip (NoC) can help provide this bandwidth.


% Optimization Fig: original workload runtime, after parallelism runtime.

% \colorbox{brown!30}{\textbf{Optimization 5:}} \textit{Hardware: reconfigurable (for sequential workload) or heterogeneous (for parallel workload) architecture supporting both neural and symbolic operations, thus can improve hardware utilization}



\subsection{Technology: Emerging Memory and Compute-In-Memory}
\label{subsec:opt_tech}
Compute-in-memory (CIM) technology~\cite{jerry2017ferroelectric,yoon202129,ankit2019puma,gomez2023evaluating,andrulis2023raella,tu202316} has been recently proposed for efficient neural network processing. We envision that neuro-symbolic computing can also be potentially accelerated with CIM as pure-VSA has been realized with taped-out CIM prototypes~\cite{li2016hyperdimensional,karunaratne2020memory}. Existing works utilize highly parallel bit-wise compute cell~\cite{kvatinsky2014magic,imani2017exploring,shou2023see} and could potentially be employed in symbolic reasoning operators such as binding/bundling/unbinding/circular convolution. Emerging non-volatile memory (eNVM) technologies can further unleash the low-power neuro-symbolic hardware with aggressive power-gating and ultra-dense memory (Mbs/mm$^2$~\cite{spetalnick202240nm,spetalnick20232}), alleviating the memory-bounded symbolic operations (Sec.~\ref{subsec:memory_roofline}). Moreover, the stochasticity of eNVM could also be exploited for better convergence performance~\cite{langenegger2023memory}. We implement an eNVM-based neuro-factorization module (NVSA components) based on CIM testchip~\cite{chang202240nm} and observe a notable gain of three orders of problem size scalability, 12.9$\times$ energy, and 5.01$\times$ area efficiency compared to digital design.

% Several NSAI workloads leverage high-dimensional representations including LTN, NVSA, and CC. Existing hardware supports for high-dimensional vectors for either matrix-vector multiplication (MVM) and bit-wise symbolic-like operations focus on macro level~\cite{imani2017exploring,shou2023see}. As we now observes the surge of high-dimensional representations~\cite{lee2023comprehensive} within NSAI workloads, efficiently breaking down the vector-symbolic operations 

\colorbox{brown!30}{\textbf{Optimization 5:}} \textit{Emerging memory technology and compute-in-memory technique can alleviate the memory-bounded symbolic operations and improve scalability, performance, area and energy efficiency of neuro-symbolic systems.}

==> Sections/8_Related_Work.tex <==
\section{Related Work}
\label{sec:related_work}

\textbf{Neural Network Characterization.}
Over the past years, computer and system architects have proposed a vast array of benchmarks, simulators, and custom architectures, most notably for characterizing and accelerating machine learning, specifically DNN training and inference across a variety of use cases ranging from mobile and edge~\cite{genesys,banbury2021mlperf,janapa2022mlperf,zhou2022ml,tambe202216,tambe202322,ramachandran2024algorithm} to large-scale cloud systems~\cite{reddi2020mlperf,mattson2020mlperf,rashidi2020astra,won2023astra}. \emph{However, neuro-symbolic systems exhibit divergent compute and memory features than DNNs and make current deep learning architecture inefficient, this paper thus takes the first step to characterize neuro-symbolic workloads to enable their efficient and scalable execution.}

\textbf{Emerging Workload Characterization.}
Beyond DNNs, benchmarks and hardware accelerators have been explored in other applications like mixed-reality~\cite{kwon2023xrbench,li2024gaze}, neuromorphic AI~\cite{yik2023neurobench,chang202373,wu2022ubrain}, robotics~\cite{wan2021energy,neuman2021robomorphic,krishnan2022roofline,liu2022energy,krishnan2022automatic,neuman2023roboshape,mayoral2023robotperf}, genome sequencing~\cite{fujiki2018genax,fujiki2020seedex}, graph~\cite{gao2023mega}, mobile vision~\cite{liu2020systolic,liu2022s2ta}, fully homomorphic execution~\cite{ma2023pytfhe,nabeel2023cofhee}, hyperdimensional computing~\cite{schlegel2022comparison,wan2024h3dfact,shou2023see}, etc. \emph{Neuro-symbolic AI shows the promising potential to be integrated into these systems and enable trustworthy applications. It is thus highly desirable to understand and optimize its system characteristics and performance.}
% Profiling emerging workloads has gained critical importance in recent times. A range of specialized benchmarking suites have been developed, including XRBench~\cite{kwon2023xrbench}, NeuroBench~\cite{yik2023neurobench}, RobotPerf~\cite{mayoral2023robotperf}, Skyline~\cite{krishnan2022roofline}, pure VSA (hyperdimensional computing, HDC)~\cite{schlegel2022comparison} and NSAI (this work). XRBench conducts profiling on real-time multi-task multi-model (MTMM) workloads. These workloads are found suitable for extended reality (XR). Compared to standard ML approach, MTMM models impose \textit{heterogeneity} and \textit{concurrency} requirements on future hardware. NeuroBench targets neuromorphic applications, striving to establish a suite of \textit{community-driven}, \textit{fair}, \textit{reproducible}, and \textit{transparent} neuromorphic benchmarks. RobotPerf presents a vendor-neutral benchmarking framework for assessing robotics computing performance across various hardware platforms, utilizing Robot Operating System-2 (ROS-2)~\cite{ros_robotics_companies}. Skyline offers an analytical benchmark to autonomous Unmanned Aerial Vehicles (UAVs), introducing a \textit{specialized roofline model} tailored for UAVs. \cite{schlegel2022comparison} surveys and profiles different VSAs, which have been adopted in NSAI back-end such as NVSA and VSAIT. The paper investigates the trade-off between the VSA vector length, accuracy, operator, similarity metric, initialization, etc. across different VSA models.



==> Sections_Old/0_Abstract.tex <==
The abstract goes here.

==> Sections_Old/1_Introduction.tex <==
\section{Introduction}

==> Sections_Old/2_Taxonomy_Workload_Application.tex <==
\section{Neurosymbolic Workload and System Requirement}
\begin{itemize}
    \item Neuralsymbolic taxonomy and workload
    \item Applications and user cases
    \item System requirement (latency, throughput, energy efficiency, etc)
\end{itemize}

==> Sections_Old/3_Profiling_Setup.tex <==
\section{Workload Characterization Methodology}
\begin{itemize}
    \item Workload profiling methodology, hardware platforms, and tools
    \item Brief description on representative neurosymbolic models used for characterization
\end{itemize}

==> Sections_Old/4_Profiling_Result.tex <==
\section{Workload Characterization Results}
\begin{itemize}
    \item Latency: breakdown, scalability
    \item Compute Operator: neuro and symbolic
    \item Memory: memory usage, cache hit/miss rate, cache throughput, DRAM BW, data transfer
    \item System: roofline analysis
    \item Neuro and symbolic interactions, data flow and control flow, identify why hardware underutilization and inefficiency
    \item Sparsity
\end{itemize}

==> Sections_Old/5_Arch_Envision.tex <==
\section{Neurosymbolic Architecture Envision}
\begin{itemize}
    \item Takeaways and opportunities from characterization
    \item What cognitive architecture for neurosymbolic workload will look like? (profiling - system/arch innovation correspondence)
    \item Transition and motivate persistent memory-centric design
\end{itemize}

==> Sections_Old/6_PM_Design.tex <==
\section{Persistence Memory Design}
Following Che-Kai's notes,
\begin{itemize}
    \item PM-centric architecture overview
    \item Macro-level design
    \item Workload scheduling (PM vs. PE)
    \item Coherence protocol for PM and PE
\end{itemize}

==> Sections_Old/7_PM_Evaluation.tex <==
\section{PM Evaluation}
\begin{itemize}
    \item Evaluation setup
    \item Evaluation results: how the design improves latency, memory, efficiency, utilization, etc. For example, through memory simulation.
\end{itemize}

==> Sections_Old/8_Outlook.tex <==
\section{Outlook and Research Opportunities}

==> Sections_Old/9_Conclusion.tex <==
\section{Conclusion}

==> Tabs/tab_algo_survey.tex <==
% \begin{table*}[]
% \resizebox{2\columnwidth}{!}{\begin{tabular}{|l|cccccll|}
% \hline
%                                                                                    & \multicolumn{7}{c|}{Neuro + Symbolic Designs}                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
%                                                                                    & \multicolumn{1}{c|}{LTN \cite{badreddine2022logic}}                & \multicolumn{1}{c|}{LNN \cite{riegel2020logical}}                                & \multicolumn{1}{l|}{NeurASP \cite{yang2020neurasp}}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Deep Orthogonal\\ Network\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Differentiable\\ ILP\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Autonomous \\ Vehicles\end{tabular}} & \multicolumn{1}{c|}{LCN \cite{marinescu2022logical}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Arbitrary\\ Queries\end{tabular}                        & \multicolumn{1}{c|}{Yes}                & \multicolumn{1}{c|}{No}                                 & \multicolumn{1}{c|}{Yes}              & \multicolumn{1}{c|}{Yes}                                                               & \multicolumn{1}{c|}{Yes}                                                          & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}Symbolic\\ Explaination\end{tabular}                    & \multicolumn{1}{c|}{No}                 & \multicolumn{1}{c|}{Yes}                                & \multicolumn{1}{c|}{Yes}              & \multicolumn{1}{c|}{No}                                                                & \multicolumn{1}{c|}{Yes}                                                          & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}Integrate Prior\\ Knowledge and Contraints\end{tabular} & \multicolumn{1}{c|}{Yes}                & \multicolumn{1}{c|}{Yes}                                & \multicolumn{1}{c|}{Yes}              & \multicolumn{1}{c|}{Yes}                                                               & \multicolumn{1}{c|}{No}                                                           & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Assures Consistency                                                                & \multicolumn{1}{c|}{No}                 & \multicolumn{1}{c|}{No}                                 & \multicolumn{1}{c|}{Yes}              & \multicolumn{1}{c|}{No}                                                                & \multicolumn{1}{c|}{No}                                                           & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Learn Rule Structure                                                               & \multicolumn{1}{c|}{No}                 & \multicolumn{1}{c|}{No}                                 & \multicolumn{1}{c|}{No}               & \multicolumn{1}{c|}{No}                                                                & \multicolumn{1}{c|}{Yes}                                                          & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Learn Classical Rules                                                              & \multicolumn{1}{c|}{No}                 & \multicolumn{1}{c|}{No}                                 & \multicolumn{1}{c|}{No}               & \multicolumn{1}{c|}{No}                                                                & \multicolumn{1}{c|}{No}                                                           & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Scalability                                                                        & \multicolumn{1}{c|}{Yes}                & \multicolumn{1}{c|}{Yes}                                & \multicolumn{1}{c|}{No}               & \multicolumn{1}{c|}{Yes}                                                               & \multicolumn{1}{c|}{No}                                                           & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Supervision                                                                        & \multicolumn{1}{l|}{Semi-supervised}    & \multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Weak Supervised}  & \multicolumn{1}{l|}{}                                                                  & \multicolumn{1}{l|}{}                                                             & \multicolumn{1}{l|}{}                                                               &                          \\ \hline
% Kautz Taxonomy                                                                     & \multicolumn{1}{l|}{$Neuro_{Symbolic}$} & \multicolumn{1}{l|}{Neuro:Symbolic $\rightarrow$ Neuro} & \multicolumn{1}{l|}{Neuro | Symbolic} & \multicolumn{1}{l|}{$Neuro_{Symbolic}$}                                                & \multicolumn{1}{l|}{Neuro:Symbolic $\rightarrow$ Neuro}                           & \multicolumn{1}{l|}{Symbolic {[}Neuro{]}}                                           &                          \\ \hline
% \end{tabular}}
% \end{table*}



\begin{table}[t!]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|}
\hline
     \textbf{\begin{tabular}[c]{@{}c@{}}NSAI Algorithms\end{tabular}}                              & \textbf{\begin{tabular}[c]{@{}c@{}}Kautz\\ Taxonomy\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}Underlying Operation \\ (Inference)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hardware\\ Scalability\end{tabular}} \\ \hline
\textbf{NVSA}  \cite{hersche2023neuro}                     & Neuro$|$Symbolic                                        & (Vec) IP and element-wise add                                                        &           Yes                                \\ \hline
\textbf{LTN} \cite{badreddine2022logic}                        & $\mbox{Neuro}_{\mbox{Symbolic}}$                        & (Vec) Fuzzy logic                                                                    &               Yes                            \\ \hline
\begin{tabular}[l]{@{}l@{}} \textbf{Differentiable ILP} \\ \cite{evans2018learning}\end{tabular}                 & \multicolumn{1}{l|}{Neuro:Symbolic $\rightarrow$ Neuro} &  (Vec) Fuzzy logic                                                                                     &         No                                  \\ \hline
\textbf{NeuPSL} \cite{pryor2022neupsl}                     & Neuro$|$Symbolic                                        & (Vec) Fuzzy logic                                                                    &                   Yes                   \\ \hline
\textbf{NeurASP} \cite{yang2020neurasp}                    & Neuro$|$Symbolic                                        &  (Non-vec)  Logic rules                                                                                 &                   No                        \\ \hline
\textbf{NS-VQA}  \cite{yi2018neural}                      & Neuro$|$Symbolic                                        & (Non-vec) Pre-defined objects                                                      &               {\color{red}No}                            \\ \hline
\textbf{LNN} \cite{riegel2020logical}                        & Neuro:Symbolic $\rightarrow$ Neuro                      & (Vec) Fuzzy logic                                                                    &             Yes                              \\ \hline
\textbf{NSCL}  \cite{maoneuro}                     & Neuro$|$Symbolic                                        & (Vec) log/sum/div/product                                                            &                 {\color{red}Yes}                          \\ \hline
\textbf{MLLR}  \cite{dai2019bridging} & Neuro$|$Symbolic                                        &    (Vec)                                                                                   &             {\color{red}No}                              \\ \hline
\textbf{SATNet}  \cite{wang2019satnet}                    &                                                         &                                                                                      &                                           \\ \hline
\textbf{NLM}   \cite{dongneural}                      & Neuro:Symbolic $\rightarrow$ Neuro                      &  (Vec)   Permutation + NN                                                                                 &                   No                        \\ \hline
\textbf{AlphaZero} \cite{silver2017mastering}                   & Symbolic{[}Neuro{]}                                     &                                                                                      & Yes                 \\ \hline
\begin{tabular}[l]{@{}l@{}}\textbf{Deep ontology networks}\\ \cite{hohenecker2020ontology}\end{tabular}     & $\mbox{Neuro}_{\mbox{Symbolic}}$                        &                                                                                      & Yes                    \\ \hline
\begin{tabular}[l]{@{}l@{}}\textbf{symbolic mathematics} \\\cite{lampledeep}\end{tabular}  & Neuro:Symbolic $\rightarrow$ Neuro          &    (Vec)  NN                                                                                &  Yes                \\ \hline
\textbf{GNN+NS}   \cite{lamb2020graph}                   & Neuro{[}Symbolic{]}                                     &                                                                                      & \multicolumn{1}{l|}{}                     \\ \hline
\end{tabular}}
\caption{NS-AI taxonomy, operation, and scalability.}
\label{tab:summary}
% \vspace{-0.5em}
\end{table}

==> Tabs/tab_temp.tex <==
% \begin{table}[t!]
% \centering
% \caption{Survey of NS-AI algorithms, operations, and scalability\vspace{3pt}.}
% \renewcommand*{\arraystretch}{1.1}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{|c|l|c|c|}
% \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Kautz\\ Taxonomy\end{tabular}}   & \multicolumn{1}{c|}{\textbf{NSAI Algorithms}}                             & \textbf{\begin{tabular}[c]{@{}c@{}}Underlying Operation \\ (Inference)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hardware\\ Scalability\end{tabular}}  \\ \hline
% \textbf{Symbolic{[}Neuro{]}}                                     & \textbf{AlphaGo} \cite{silver2017mastering}                   &                                                                                      & Yes                 \\ \hline
% \multirow{6}{*}{\textbf{Neuro$|$Symbolic}} & \textbf{NVSA}~\cite{hersche2023neuro}  & (Vec) IP and element-wise add                                                        &           Yes \\ \cline{2-4} 
%                    & \textbf{NeuPSL} \cite{pryor2022neupsl}   & (Vec) Fuzzy logic                                                                    &                   Yes    \\ \cline{2-4} 
%                    & \textbf{NeurASP} \cite{yang2020neurasp} & (Non-vec)  Logic rules                                                                                 &                   No \\ \cline{2-4} 
%                    & \textbf{NSCL}  \cite{maoneuro} & (Vec) log/sum/div/product                                                            &                 {\color{red}Yes} \\ \cline{2-4} 
%                    & \textbf{MLLR}  \cite{dai2019bridging} & (Non-vec) Logic rules                                                                                 &             {\color{red}No}  \\ \cline{2-4} 
%                    & \textbf{NSVQA}  \cite{yi2018neural}  & (Non-vec) Pre-defined objects                                                      &               {\color{red}No} \\ \hline
% \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}\textbf{Neuro:Symbolic}\\ \textbf{$\rightarrow$Neuro}\end{tabular}} & \textbf{LNN} \cite{riegel2020logical}  & (Vec) Fuzzy logic                                                                    &             Yes \\ \cline{2-4} 

%                    & \begin{tabular}[l]{@{}l@{}}\textbf{Symbolic Mathematics} \\ \cite{lampledeep}\end{tabular} & (Vec)  NN                                                                            &  Yes \\ \cline{2-4} 
                   
%                    & \begin{tabular}[l]{@{}l@{}}\textbf{Differentiable ILP}\\ \cite{evans2018learning}\end{tabular} & (Vec) Fuzzy logic                                                                                     &         No \\ \hline
% \multirow{2}{*}{\textbf{$\mbox{Neuro}_{\mbox{Symbolic}}$ }} & \textbf{LTN} \cite{badreddine2022logic}  & (Vec) Fuzzy logic                                                                    &               Yes \\ \cline{2-4} 
%                    & \begin{tabular}[l]{@{}l@{}}\textbf{Deep ontology networks}\\ \cite{hohenecker2020ontology}\end{tabular}  & (Vec) NN  & Yes  \\ \hline
% \multirow{3}{*}{\textbf{Neuro{[}Symbolic{]}} }                  & \begin{tabular}[l]{@{}l@{}}\textbf{GNN+attention}\\ \cite{lamb2020graph}\end{tabular} & (Vec) SpMM + SDDMM & Yes\\ \cline{2-4} 
% & \textbf{NLM} \cite{dongneural}  &  (Vec)   Permutation + NN          &    No \\ \cline{2-4} 
%                   & \textbf{SATNet}  \cite{wang2019satnet} &  & Yes \\ \hline
% \end{tabular}}
% \label{tab:summary}
% \vspace{-15pt}
% \end{table}

\begin{table}[t!]
% \vspace{-7pt}
\centering
% \caption{Survey of recent NSAI algorithms into five categories, each with summarized underlying operations and vector formats\vspace{3pt}.}
\caption{Review of recent neuro-symbolic AI algorithms into five categories, with their underlying operations and vector formats.}
\renewcommand*{\arraystretch}{1.15}
\setlength\tabcolsep{1.8pt}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Category\end{tabular}}   & \multicolumn{1}{c|}{\textbf{Neuro-Symbolic Algorithm}}                             & \textbf{\begin{tabular}[c]{@{}c@{}} Underlying Operation\end{tabular}} & \multicolumn{1}{c}{\textbf{If Vector}}                \\ \hline
\textbf{Symbolic{[}Neuro{]}}                                     & \textbf{AlphaGo} \cite{silver2017mastering}     &    NN, MCTS                                                                                  & Vector                 \\ \hline
\multirow{8}{*}{\textbf{Neuro$|$Symbolic}} & \textbf{NVSA}~\cite{hersche2023neuro}  & NN, mul, add, circular conv.       &   Vector \\ \cline{2-4} 
                   & \textbf{NeuPSL} \cite{pryor2022neupsl}   &  NN, fuzzy logic      &              Vector  \\ \cline{2-4} 
                & \textbf{NSCL}  \cite{maoneuro} & NN, add, mul, div, log    &      Vector \\ \cline{2-4} 
                   & \textbf{NeurASP} \cite{yang2020neurasp} &  NN, logic rules     &   Non-Vector \\ \cline{2-4} 
                   & \textbf{ABL}  \cite{dai2019bridging} &NN, logic rules    &       Non-Vector \\ \cline{2-4} 
                   & \textbf{NSVQA}  \cite{yi2018neural}  &  NN, pre-defined objects      &     Non-Vector \\ \cline{2-4}
                   & \textbf{VSAIT}  \cite{theiss2022unpaired}  &  NN, binding/unbinding    & Vector \\ \cline{2-4} 
                   & \textbf{PrAE}  \cite{zhang2021abstract}  &  NN, logic rules, prob. abduction      &  Vector \\ \hline


                   
\multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}\textbf{Neuro:Symbolic}\\ \textbf{$\rightarrow$Neuro}\end{tabular}} & \textbf{LNN} \cite{riegel2020logical}  &  NN, fuzzy logic               & Vector\\ \cline{2-4} 

                   & \begin{tabular}[l]{@{}l@{}}\textbf{Symbolic Math}~\cite{lampledeep}\end{tabular} &  NN                                                                            & Vector \\ \cline{2-4} 
                   
                   & \begin{tabular}[l]{@{}l@{}}\textbf{Differentiable ILP}~\cite{evans2018learning}\end{tabular} &  NN, fuzzy logic                                                                                     & Vector \\ \hline
\multirow{2}{*}{\textbf{$\mbox{Neuro}_{\mbox{Symbolic}}$ }} & \textbf{LTN} \cite{badreddine2022logic}  & NN, fuzzy logic                                                                    & Vector \\ \cline{2-4} 
                   & \begin{tabular}[l]{@{}l@{}}\textbf{DON}~\cite{hohenecker2020ontology}\end{tabular}  & NN  & Vector  \\ \hline
\multirow{3}{*}{\textbf{Neuro{[}Symbolic{]}} }                  & \begin{tabular}[l]{@{}l@{}}\textbf{GNN+attention}~\cite{lamb2020graph}\end{tabular} & NN, SpMM, SDDMM & Vector\\ \cline{2-4} 
& \textbf{ZeroC} \cite{wu2022zeroc}  & NN (energy-based model, graph)& Vector \\  \cline{2-4} 
& \textbf{NLM} \cite{dongneural}  &  NN, permutation         &  Vector \\  \hline
                  % & \textbf{SATNet}  \cite{wang2019satnet} &  & Yes \\ \hline
\end{tabular}}
\label{tab:summary}
\vspace{-5pt}
\end{table}
